Syntax-Guided Program Reduction for Understanding Neural Code Intelligence Models

Neural code intelligence (CI) models are opaque black-boxes and offer little insight on the features they use in making predictions. This opacity may lead to distrust in their prediction and hamper their wider adoption in safety-critical applications. Recently, input program reduction techniques have been proposed to identify key features in the input programs to improve the transparency of CI models. However, this approach is syntax-unaware and does not consider the grammar of the programming language. In this paper, we apply a syntax-guided program reduction technique that considers the grammar of the input programs during reduction. Our experiments on multiple models across different types of input programs show that the syntax-guided program reduction technique is faster and provides smaller sets of key tokens in reduced programs. We also show that the key tokens could be used in generating adversarial examples for up to 65% of the input programs.

==> resources/methodname.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{resources/images/swap.png}
    \caption{An example of \mnp task by \ctv\cite{alon2019code2vec}.}
    \label{fig:example}
    %\vspace{-1mm}
\end{figure}


==> resources/models.tex <==
\begin{table}
    \begin{center}
        \caption{Performance of the CI models on test set.}
        \def\arraystretch{1.23}
        \label{table:ci_models}
        \resizebox{0.95\columnwidth}{!}{%
        \begin{tabular}{|c|c|c|c|c|}
            \hline
            \textbf{Model} & \textbf{Dataset} & 
            \textbf{Precision} & \textbf{Recall} & \textbf{$F_1$-Score} \\ \hline 
            \hline
            \ctv & \multirow{2}{*}{\JL} & 45.17 & 32.28 & 37.65 \\ \cline{1-1} \cline{3-5}
            \cts & & 64.03 & 55.02 & 59.19 \\ \hline 
        \end{tabular}%
        }
    \end{center}
\end{table}


==> settings.tex <==
\section{Implementation}

To implement and evaluate our approach, we study two well-known code intelligence models (\ctv and \cts), a popular code intelligence task (\mnp) and one commonly used programming language dataset (\JL) with different type input programs. However, our approach can be applicable to other models, tasks, and programming languages.


\subsection{Task:}
We use the popular code intelligence task: method name prediction (\mnp \cite{allamanis2015suggesting}) in this study. This task is commonly used by researchers in the code intelligence domain for various applications such as code summarization \cite{allamanis2015suggesting,allamanis2016summarization}, representation learning \cite{alon2019code2vec,alon2019code2seq}, neural testing \cite{kang2019generalizability,yefet2020adversarial,rabin2021generalizability}, feature extraction \cite{rabin2021sivand,wang2021demystifying}, and so on \cite{allamanis2018bigcode, allamanis2019duplication}.
In this \mnp task, a model attempts to predict the name of a method from its body. For example, given the following code snippet: ``\texttt{void f(int a, int b) \{int temp = a; a = b; b = temp;\}}'', a model aims to predict the method's name as ``\texttt{swap}''.





\subsection{Model:}
We use two well-known \ci models for \mnp task: \ctv~\cite{alon2019code2vec} and \cts~\cite{alon2019code2seq}. Both models use paths from abstract syntax trees (AST) to encode a program.
\begin{itemize}
    \item \ctv. This model extracts a bag of path-context from the AST of the program where each path-context includes a pair of terminal nodes and the corresponding path between them. The model learns embeddings of these path-contexts during training and uses an attention mechanism to aggregate multiple path-contexts to a single code vector. The code vector is used as a representation of the program for making a prediction.
    \item \cts. This model also extracts a bag of path-context from the AST of the program but it sub-tokenized each path-context. The \cts model uses a bi-directional LSTM to encode paths node-by-node, and another LSTM to decode a target sequence one-by-one.
\end{itemize}
Using \texttt{JavaExtractor} of \ctv and \cts models, we extract and preprocess the bag of path-contexts from Java files. For example, given a sample expression: ``\texttt{tempVar = 0;}'', a path-context by \ctv is: ``\texttt{tempVar, <NameExpr ↑ AssignExpr ↓ IntegerLiteralExpr>, 0}'' and a path-context by \cts is: ``\texttt{temp|var, NameExpr | AssignExpr | IntegerLiteralExpr, 0}''.

\subsection{Dataset}
For the \mnp task, we use the \JL dataset \cite{alon2019code2seq}. This dataset contains a total of $9,500$ Java projects from GitHub, where $9,000$ projects are for the training set, $200$ projects for the validation set, and $300$ projects for the test set. Using training set and validation set, we train both the \ctv and \cts models. Table ? summarizes the performance characteristics of these models.

\subsection{Input Types}
The dataset from GitHub is often imbalanced and contains different sizes and frequencies of input programs. Therefore, to evaluate the effectiveness of our approach, we choose different type of input programs from \JL test set.

\begin{itemize}
    \item Frequent Methods: We randomly sample a total of $100$ input programs from the most occurring method names.
    \item Rare Methods: We randomly sample a total of $100$ input programs from the least occurring method names.
    \item Smaller Methods: We randomly sample a total of $100$ input programs that contains less than $10$ lines of code.
    \item Larger Methods: We randomly sample a total of $100$ input programs that has around $100$ lines of code.
\end{itemize}

